Automatically Generating Questions About Scratch Programs

When learning to program, students are usually assessed based on the code they wrote. However, the mere completion of a programming task does not guarantee actual comprehension of the underlying concepts. Asking learners questions about the code they wrote has therefore been proposed as a means to assess program comprehension. As creating targeted questions for individual student programs can be tedious and challenging, prior work has proposed to generate such questions automatically. In this paper we generalize this idea to the block-based programming language Scratch. We propose a set of 30 different questions for Scratch code covering an established program comprehension model, and extend the LitterBox static analysis tool to automatically generate corresponding questions for a given Scratch program. On a dataset of 600,913 projects we generated 54,118,694 questions automatically. Our initial experiments with 34 ninth graders demonstrate that this approach can indeed generate meaningful questions for Scratch programs, and we find that the ability of students to answer these questions on their programs relates to their overall performance.

==> tables/block_model_instances.tex <==
\begin{table}
\centering
\caption{Number of questions generated per Block Model cell, standardized by 
number of questions per cell.}
\label{block_model_instances}
\sffamily
\small
\begin{tabularx}{\columnwidth}{>{\color{white}\columncolor[gray]{.4}}lXXX}
%\toprule
\rowcolor[gray]{.4}  & \color{white}Text & \color{white} Execution & \color{white} Purpose \\
%\midrule
\rotatebox[origin=c]{90}{\begin{minipage}[c]{1cm}\centering{}Atom\end{minipage}}  &    \atomTextNorm & \atomExecutionNorm & \atomPurposeNorm \\
\rotatebox[origin=c]{90}{\begin{minipage}[c]{1cm}\centering{}Block\end{minipage}}  & \blockTextNorm & \blockExecutionNorm & \blockPurposeNorm \\
\rotatebox[origin=c]{90}{\begin{minipage}[c]{1cm}\centering{}Relation\end{minipage}} & \relationTextNorm & \relationExecutionNorm & \relationPurposeNorm \\
\rotatebox[origin=c]{90}{\begin{minipage}[c]{1cm}\centering{}Macro\end{minipage}} & \macroTextNorm & \macroExecutionNorm & \macroPurposeNorm \\
              
%\bottomrule
\end{tabularx}
\end{table}


==> tables/data_block_model_sum.tex <==
\begin{table}
\centering
\caption{Number of questions instances found per Block Model cell.}
\label{instances_per_block_model}
\begin{tabular}{lr}
\toprule
{} &         0 \\
\midrule
Atom Text          &   6595576 \\
Atom Execution     &   2199143 \\
Atom Purpose       &   6694025 \\
Block Text         &   2774687 \\
Block Execution    &   5118361 \\
Block Purpose      &  15102402 \\
Relation Text      &   2073706 \\
Relation Execution &   3508034 \\
Relation Purpose   &   1103245 \\
Macro Text         &   6529933 \\
Macro Execution    &   1818669 \\
Macro Purpose      &    600913 \\
\bottomrule
\end{tabular}
\end{table}

